Learning Lightweight Lane Detection CNNs by Self Attention Distillation

Training deep models for lane detection is challenging due to the very subtle and sparse supervisory signals inherent in lane annotations. Without learning from much richer context, these models often fail in challenging scenarios, e.g., severe occlusion, ambiguous lanes, and poor lighting conditions. In this paper, we present a novel knowledge distillation approach, i.e., Self Attention Distillation (SAD), which allows a model to learn from itself and gains substantial improvement without any additional supervision or labels. Specifically, we observe that attention maps extracted from a model trained to a reasonable level would encode rich contextual information. The valuable contextual information can be used as a form of 'free' supervision for further representation learning through performing topdown and layer-wise attention distillation within the network itself. SAD can be easily incorporated in any feedforward convolutional neural networks (CNN) and does not increase the inference time. We validate SAD on three popular lane detection benchmarks (TuSimple, CULane and BDD100K) using lightweight models such as ENet, ResNet-18 and ResNet-34. The lightest model, ENet-SAD, performs comparatively or even surpasses existing algorithms. Notably, ENet-SAD has 20 x fewer parameters and runs 10 x faster compared to the state-of-the-art SCNN, while still achieving compelling performance in all benchmarks. Our code is available at https://github.com/cardwing/Codes-for-Lane-Detection.

==> general.tex <==

Since lane detection demands real-time performance ($>$ 20 fps) in real-world applications while most conventional methods fail to fulfill this requirement due to the deployment of deep models like VGG-16~\cite{simonyan2014very} or ResNet-101~\cite{he2016deep}, we consider to use light-weight models as our backbones, i.e., ENet~\cite{paszke2016enet}, ResNet-18~\cite{he2016deep} and ResNet-34~\cite{he2016deep}. Note that we replace the original spatial max unpooling module in ENet with bilinear upsampling followed by 1$\times$1 convolution since we empirically find that this modification can improve the overall performance. Besides, ENet is an encoder-decoder structure and therefore the output probability maps are the same size as the input image. As to ResNet-18 and ResNet-34, they work as an encoder and their output probability maps are 8 $\times$ smaller resolutions compared with original images. Following ~\cite{pan2017spatial}, we use bilinear upsampling to recover the original image size. However, due to the lack of a specifically designed decoder module, ResNet-18 and ResNet-34 perform poorer than ENet although they have much more parameters than ENet. Therefore, we choose to use ENet\footnote{URL of model and codes will be provided after peer review.} as our final backbone and ResNet-18 and ResNet-34 are only used to validate the effectiveness and generality of our proposed techniques. Fig. \ref{fig:pipeline} depicts the basic architecture of our ENet model. Note that the three components in A denote the three blocks of the ENet encoder and two components in B are two blocks in the decoder.   

\begin{figure*}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{./figure/framework.pdf}
  \vskip -0.2cm
  \caption{Illustration of ENet-\algorithmname. $E_{1}$ $\sim$ $E_{4}$ comprise the encoder, $D_{1}$ and $D_{2}$ comprise the decoder and $P_{1}$ denotes the small network used to predict the existence of lanes.}
  \centering
  \label{fig:pipeline}
\end{figure*}

\subsection{Dataset}

\begin{table*}[!t]
\caption{A brief description about three lane detection datasets.}
\label{dataset_table}
\centering
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline
Name & \# Frame & Train & Validation & Test & Resolution & Road Type & \# Lane $>$ 5 ? \\
\hline
TuSimple & 6, 408 & 3, 626 & -- & 2, 782 & 1280 $\times$ 720 & highway & $\times$ \\
\hline
CULane & 133, 235 & 88, 880 & 9, 675 & 34, 680 & 1640 $\times$ 590 & urban, rural and highway & $\times$ \\
\hline
BDD100K & 80, 000 & 70, 000 & -- & 10, 000 & 1280 $\times$ 720 & urban, rural and highway &  $\surd$ \\
\hline
\end{tabular}
\end{table*}

\begin{figure}[t]
  \centering
  \includegraphics[width=1.0\linewidth]{./figure/dataset.pdf}
  \vskip -0.2cm
  \caption{Typical video frames of TuSimple, CULane and BDD100K datasets.}
  \centering
  \label{fig:dataset}
\end{figure}

Table \ref{dataset_table} records the basic information of three lane detection datasets. Note that the last column of Table \ref{dataset_table} shows that TuSimple and CULane have no more than 5 lanes in a video frame while BDD100K typically has more than 8 lanes in a video frame. Besides, TuSimple is relatively easy while CULane and BDD100K are more challenging considering the total number of video frames and road types. Note that original BDD100K dataset provides 100 k video frames, 70 k for training, 10 k for validation and 20 k for testing. However, since they do not provide ground-truth labels for testing set, we keep the training set unchanged but use the original validation set for testing.   


\subsection{Evaluation Criterion}

\noindent \textbf{TuSimple:} in TuSimple, we use the official metric (accuracy) as the evaluation criterion. Besides, false positive ($FP$) and false negative ($FN$) are also listed. The following is the equation to compute accuracy~\cite{tusimple}: 

\begin{equation}
Accuracy = \frac{N_{pred}}{N_{gt}} ,
\end{equation}

where $N_{pred}$ is the number of correctly predicted lane points and $N_{gt}$ is the number of ground-truth lane points.

\noindent \textbf{CULane and BDD100K:} to judge whether a lane is correctly detected, we treat each lane as a line with fixed pixel width (30 for CULane and 8 for BDD100K) and compute the intersection-over-union (IoU) between labels and predictions. Predictions whose IoUs are larger than 0.5 are considered as true positives (TP). Then, we use $F_{1}-measure$ as the evaluation metric formulated as follows:

\begin{equation}
F_{1}-measure = \frac{2 \times Precision \times Recall}{Precision + Recall} ,
\end{equation}

where $Precision = \frac{TP}{TP + FP}$ and $Recall = \frac{TP}{TP + FN}$.


\subsection{Methods}

We give a brief introduction to several CNN-based lane detection models. Note that the following approaches all adopt the encoder and decoder structure as the main network.

\noindent \textbf{SCNN:} SCNN uses VGG-16 as the encoder, bilinear upsampling as the decoder and performs message passing to better exploit the long, thin prior of lanes. Besides, the lane existence prediction branch is added to provide extra performance gains as well as facilitate the evaluation process.  

\noindent \textbf{ResNet-101:} similar to SCNN except that the encoder is ResNet-101 and no message passing is used, it achieves compelling performance in CULane. 

\noindent \textbf{LaneNet:} it is mainly comprised of two sub-networks, i.e., LaneNet and H-Net. The former is used to generate the segmentation maps differentiating lane instances and background. The later is utilized to obtain the lane points from original images and segmentation maps to facilitate evaluation.

\noindent \textbf{EL-GAN:} it adopts U-Net~\cite{ronneberger2015u} as the generator (i.e., the encoder and decoder) and DenseNet~\cite{huang2017densely} as the discriminator. The introduction of GAN aims at generating more realistic segmentation maps as well as easing the complex post-processing.

\noindent \textbf{GC-LD:} it uses VGG-16 as the backbone and performs lane and road detection simultaneously. Both geometric prior and inner relationship between two detection tasks are exploited to boost the overall performance of their models.
